Sensitivity of Trapping Efficiency and Relative Permeability to Experimental Methodology in Laboratory Core Flooding

Understanding the migration and trapping of CO$_2$ in the subsurface is vital to geologic carbon storage projects. Traditional characterization methods employ steady-state co-injection experiments to determine relative permeability and trapping efficiency. Although laboratory studies aim to replicate reservoir conditions, co-injection experiments are often selected because they facilitate steady-state flow and reduce capillary end effects. The fundamental influence of this experimental design choice on measured petrophysical parameters remains inadequately characterized. This study presents a comparative analysis between co-injection and single-phase injection experiments, specifically investigating how experimental methodology influences both trapping efficiency and pressure differential across the core sample (which is used to calculate relative permeability). Our results demonstrate significant variations in trapping behavior between these injection techniques, suggesting that the traditional focus on co-injection experiments may overlook important physical flow phenomena. Differences between injection techniques could be strategically exploited in field applications to enhance residual trapping capacity in subsurface CO$_2$ storage operations. This work highlights the importance of understanding experimental artifacts in core flooding studies and their potential applications for improving carbon storage efficiency.

==> CHAPTERS/intro.tex <==
\section{Introduction}

The storage of CO$_2$ in porous subsurface rocks (geologic carbon sequestration) is integral to mitigating climate change \cite{ipcc2014, bui2018carbon, benson2012carbon}. Understanding the migration and trapping of CO$_2$ in subsurface reservoirs is vital to ensuring the safe, long-term storage. The trapping of CO$_2$ by capillary forces, or residual trapping, is an important mechanism for maximizing storage capacity and guaranteeing the long term storage of CO$_2$ underground \cite{krevor2015capillary}. Maximizing the amount of CO$_2$ trapped by this mechanism will minimize plume spread, and increase plume immobilization, thus increasing storage capacity and security \cite{krevor2015capillary, krevor2011capillary}. 

Reservoir models are used to predict the propagation and trapping of CO$_2$ underground \cite{ringrose2013salah, bentham2005co2, ampomah2016evaluation}. Key inputs for these models are relative permeability, capillary pressure and trapping curves (the relationship between initial gas saturation and residual gas saturation). These properties are measured on core/cm-scale samples, and assumed to be representative of larger scale systems. In fact, experiments are often conducted at high temperatures and pressures to represent reservoir conditions, so that they are more representative of subsurface conditions \cite{krevor2016impact, selem2021pore, singh2018partial}. These experiments are time consuming and expensive. While reservoir conditions are created in the core, typically steady-state experiments with the co-injection of both phases are conducted because capillary end effects are less prominent \cite{pini2017capillary, bertels2001measurement, avraam1995flow}. Capillary end effects are a strong saturation gradient caused by the gas preferentially leaving the core and occupying the metal end piece. Other methods to discount the end efforts have included removing the end section from analysis \cite{pini2017capillary,perrin2010experimental}, correcting for end effects prior to analysis \cite{archer1973use, jackson2018characterizing, krause2015accurate, reynolds2018multiphase}, and adding a porous plate or other rock core in sequence to the rock of interest \cite{honarpour1988relative, avraam1995flow, persoff1995two}.



Steady-state co-injection experiments have been shown to have different underlying pore scale dynamics than unsteady-state co-injection experiments, with the unsteady-state dynamics leading to more mobile CO$_2$ \cite{spurin2020real}. However, it is typical to do steady-state co-injection experiments, and use the same values for the whole plume, regardless of the dynamics expected. It is also assumed that the residual trapping measured in these experiments can be used to parameterize models for hysteresis in relative permeability and capillary pressure constitutive functions \cite{krevor2015capillary}. With unsteady-state and steady-state co-injection experiments showing distinct behaviour. The difference before co-injection experiments, where both fluids are injected simultaneously, and single phase injection experiments, where a single fluid is injected, must be understood. Furthermore, by removing the end of the core from the analysis, we potentially remove the drop in saturation caused by the capillary end effect. However, this does not remove the role of the end effect in the pressure data used to calculate relative permeability, and can lead to incorrect relationships between saturation and pressure. Corrections for capillary end effects have been successfully applied to homogeneous sandstone samples, but they have failed to correct end effects in heterogeneous sandstone and carbonate samples \cite{manoorkar2021observations, wenck2021simulating}. Thus the link between heterogeneities and capillary discontinuities is still missing. A porous plate, or additional rock core can reduce end effects. But, as with cropping, it does not untangle the role of end effects in the pressure data, instead the properties of the other samples or porous plate are now included. 



If we are unaware of the constraints of an experiment or the difference between different injection techniques, then utilising the data at the field scale will lead to large uncertainties. With single phase injection more likely for the application of CO$_2$ storage, we need to understand the impact of different injection techniques on the fluid dynamics, and understand the influence of the injection technique on the residual trapping of CO$_2$. If we are investing significant time and effort into conducting core-scale experiments to understand large scale dynamics, we must be certain that the experiments are representative of what is occurring at the larger scale. In this work, we present the difference between single phase flow experiments and co-injection experiments for two fluid pairings: gas and water, and oil and water. We use the two fluid pairings to highlight how the dynamics differ between CO$_2$ storage, and conventional oil recovery to provide insight into the changes required for reservoir modelling for applications of carbon storage. 




==> CHAPTERS/methods.tex <==
\section{Materials and Methods}
\subsection{Rocks} 
A cylindrical Indiana limestone sample, 5 cm in diameter and 12 cm in length was used in this work. The same sample was used in all experiments, with the porosity along the core increasing slightly with distance along the core, as shown in Figure \ref{porosity}. %For the oil/water experiments, different Indiana samples were used, as removing oil from the system is time-consuming and difficult, with any remaining oil would affect the trapping curves presented in this work. 
Indiana is a heterogeneous limestone with a bimodal porosity distribution; the heterogeneities manifest at the mm scale, which is below the resolution of the images acquired in this work \cite{manoorkar2021observations}.

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.8\linewidth]{CHAPTERS/PICS/porosity.png}
	\end{center}
	\caption{Porosity profile for the Indiana core for the initial orientation. Experiments are also performed with the inlet and outlet switched. In these experiments the higher porosity is at the inlet.}
	\label{porosity}
\end{figure}

%\textcolor{red}{Insert the porosity profiles of the other oil/water experiments}

\subsection{Fluids, Interfacial Tension and Viscosity}
%Two fluid pairings were used in this work: gas and water, and oil and water. 

The non-wetting phase for these experiments was nitrogen, and the wetting phase was deionised water. Nitrogen was used as a proxy for CO$_2$ because it has a similar viscosity and density (so the residual trapping is expected to be the same \cite{wildenschild2011exploring}), but a much lower miscibility with water. Using nitrogen allowed us to explore a gas/water system (analogous to CO$_2$ injection into a saline aquifer) while minimizing dissolution (which is beyond the scope of this research). The properties of the chosen fluids is listed Table \ref{fluid_properties}.

\begingroup
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\begin{table}[]
\caption{The properties of the non-wetting phase (nitrogen) and wetting phase (water) used in this work.}
\begin{tabular}{@{}ccc@{}}
\hline
\multicolumn{1}{c}{Fluid} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Viscosity, $\mu$\\ (Pa.s)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Interfacial tension \\ with water, $\sigma$\ (N/m)\end{tabular}} \\ \hline
Nitrogen                  & $2.08 \times 10^{-5}$                                                                & $64 \times 10^{-3}$                                                                                                             \\
%Decane                    & $83.8 \times 10^{-5}$                                                                & $47 \times 10^{-3}$                                                                                                           \\
Water                     & $95.0 \times 10^{-5}$                                                                & N/A                                                                                                                           \\ \hline
\end{tabular}
\label{fluid_properties}
\end{table}
\endgroup



\subsection{Experimental procedure \& Image processing} 
Two injection methods were explored in this work:single phase injection and co-injection. Prior to any injection, the sample was loaded into a core holder that allows pressurisation of the fluids, and placed in the medical CT scanner used to image the core and the fluid distributions within. A confining pressure was applied that was always 2~MPa above the pressure in the core. Then 2 consecutive scans were taken to capture the rock with only air occupying the pore space. These scans were averaged to improve image quality \cite{pini2016moving, kurotori2023mixed}. This gives $CT_{ar}$, which is the CT number of the core filled with air. Then the core was then saturated with deionized water and pressurized to 8~MPa. Another 2 scans were acquired, and averaged to get $CT_{wr}$, which is the CT number of the core filled with water. From these images, the porosity ($\phi$) across the core was calculated using: 


\begin{equation}
\phi = \frac{CT_{wr} - CT_{ar}}{CT_{water} - CT_{air}}
\end{equation}

where $CT_{water}$ = 0 is the CT number of the pure water phase, and $CT_{air}$ = -1000 is the CT number of the pure air phase at atmospheric pressure and room temperature \cite{akin2003computed}. 


For the single phase injection experiments, a drainage sequence was performed first, with the non-wetting phase injected at a constant flow rate until 300 ml of fluid had been injected. The flow rates are given in Table \ref{flow_rates}, and were chosen to ensure flow was in the capillary dominated regime. Then an imbibition sequence was performed, with water injected at a constant flow rate until 300 ml of fluid had been injected. CT imaging occurred during flow, and at the end of both the drainage and imbibition cycles. 

For the co-injection experiments, a drainage sequence was performed first with both fluids injected at a constant flow rate, and fractional flow, until 300 ml of the non-wetting fluid had been injected. Then an imbibition sequence was performed, with both phases injected again, but the water constituting the majority of the total flow rate, until 300 ml of the wetting fluid had been injected, to allow comparable trapping relationships between the experiments. The flow rates chosen are given in Table \ref{flow_rates}. CT imaging occurred during flow, and at the end of both the drainage and imbibition cycles. 


The resolution of the CT images was 1~mm$^3$ per voxel. This means that fluid interfaces themselves cannot be resolved but the saturation could be calculated at the voxel level using: 

\begin{equation}
    S_g = \frac{CT_{flow} - CT_{satwr}}{\phi }.
    \label{sat_with_porosity}
\end{equation}



Further details on the analysis of medical CT imaging is given in \citet{akin2003computed, krevor2012relative, pini2016moving, kurotori2019measuring}. 


Between experiments the core was depressurised and flushed with water, before the system was re-pressurised. This removes gas from the system, as confirmed by the wet scans prior to an experiment.



\begingroup
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\begin{table}[]
\caption{The flow rates chosen for the different experiments, with the injected volume of the non-wetting phase (NWP) kept constant for the drainage experiments at 300ml. The capillary number for the experiments is also given.}
\begin{tabular}{@{}ccccc@{}}
\hline
{Experiment} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}NWP flow rate\\ (ml/min)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Water flow rate\\ (ml/min)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Duration\\ (mins)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Capillary \\ number\end{tabular}} \\ \hline
Gas/ water single phase drainage          & 5                                                                                              & 0                                                                                                & 60                                                                                      & $1.4 \times 10^{-8}$                                                                      \\ \hline
Gas/ water single phase imbibition        & 0                                                                                              & 5                                                                                                & 60                                                                                      & $6.0 \times 10^{-7}$                                                                      \\ \hline
Gas/ water co-injection drainage          & 5                                                                                              & 1                                                                                                & 60                                                                                      & $2.0 \times 10^{-8}$                                                                      \\ \hline
Gas/ water co-injection imbibition        & 1                                                                                              & 5                                                                                                & 60                                                                                      & $8.9 \times 10^{-8}$                                                                      \\ \hline
%Oil/ water single phase drainage          & 3                                                                                              & 0                                                                                                & 100                                                                                     & $4.5 \times 10^{-7}$                                                                      \\ \hline
%Oil/ water single phase imbibition        & 0                                                                                              & 3                                                                                                & 100                                                                                     & $4.9 \times 10^{-7}$                                                                      \\ \hline
%Oil/water co-injection drainage           & 3                                                                                              & 0.6                                                                                              & 100                                                                                     & $5.5 \times 10^{-7}$                                                                      \\ \hline
%Oil/ water co-injection imbibition        & 0.6                                                                                            & 3                                                                                                & 100                                                                                     & $5.8 \times 10^{-7}$                                                                      \\ \hline
\end{tabular}
\label{flow_rates}
\end{table}
\endgroup


==> CHAPTERS/results.tex <==
\section{Results and discussion}
%submit to transport in porous media 

\subsection{Saturation along the core after drainage and imbibition}
\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.95\linewidth]{CHAPTERS/PICS/sat_n2.png}
	\end{center}
	\caption{Saturation along the core after drainage (black) and imbibition (red) for a) the co-injection experiments and b) the single phase injection experiments.}
	\label{sat_n2}
\end{figure}

Figure \ref{sat_n2} shows the saturation along the core at the end of drainage and at the end of imbibition with the co-injection experiment plotted in a) and the single phase injection experiment plotted in b). Saturation after drainage is significantly higher for the single phase injection experiment, whereas, saturation after imbibition is similar for both experiments. This means that the difference between drainage and imbibition is larger for the single phase injection experiment. The saturation profiles suggest key differences between the injection scenarios that will be reflected in the residual trapping efficiency. 

At the end of imbibition, there is evidence for capillary end effects for both experiments, shown by the decrease in gas saturation towards the outlet of the core. The influence of the capillary end effect extends to approximately half the core (6 cm) in both cases, but is evidently more extreme for the single phase injection experiment, with the gas saturation dropping to zero at approximately 8 cm from the inlet, whereas for the co-injection experiment, the gas saturation drops, but not to zero. Overall, capillary end effects exist for both types of experiments at the end of imbibition. However, they are more extreme when there is no gas injection to maintain flow pathways i.e. during single phase injection. The drop to zero saturation at the end of the core heavily influences the pressure drop across the core, which is discussed in Section \ref{pressure}. 

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.95\linewidth]{CHAPTERS/PICS/sat_poro_n2.png}
	\end{center}
	\caption{The relationship between saturation and porosity for each slice in the core. The black crosses denote drainage, and the red circles denote imbibition for a) the co-injection experiment and b) the single phase injection experiment.}
	\label{sat_poro_n2}
\end{figure}

There is a less significant drop in gas saturation towards the outlet of the core at the end of drainage (when compared to the end of imbibition) for the co-injection experiment. However, for the single phase injection experiment, gas saturation increases towards the inlet. The relationship between saturation and porosity is shown in Figure \ref{sat_poro_n2} a) for the co-injection experiment, and b) for the single phase injection experiment. At the end of single phase drainage is the only case where there is a positive correlation between gas saturation and porosity. For all other cases, there is a negative correlation between gas saturation and porosity. The rock sample is assumed to be water-wet, thus the gas (as the non-wetting phase) is expected to occupy the larger pores, leading to a positive correlation between gas saturation and porosity. However, for this sample there is a very slight increase in porosity with distance from the inlet i.e. the porosity is correlated with distance along the core; this is shown in Figure \ref{porosity}. The capillary end effect opposes the relationship expected from the porosity gradient, and is a stronger signal, thereby influencing the porosity-saturation relationship throughout the core. This suggests that analyses that “crop” the end effects out, will still be influenced by the end effects. Thus we need to understand the impact of capillary end effects on trapping in order to successfully apply core scale experiments to subsurface reservoir models. End effects must be carefully considered if one is using porosity-saturation relationships to deduce the wettability of the core.


\subsection{Trapping curves}
The trapping curves (Figure \ref{trapping_curve}) highlight the fundamental difference between the different injection techniques, and the potential errors that can arise from not considering the impact of the chosen injection technique on residual trapping. The result from the co-injection experiment agrees with previous experimental observations by \citet{niu2015impact}, where the the slice-by-slice analysis can be fitted with a single Land trapping model. The authors argued that the end effects could be exploited as they increased the saturation range for the trapping curve, making the interpretation of the data with a Land trapping model more reliable. However, for the single phase injection experiments, the end effects create distinct regions that cannot be modelled with a single Land trapping curve. 

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.8\linewidth]{CHAPTERS/PICS/trapping_curve.png}
	\end{center}
	\caption{The relationship between between initial gas saturation (post drainage) and residual gas saturation (post imbibition) for the co-injection experiment (black crosses) and single phase injection experiment (red circles).}
	\label{trapping_curve}
\end{figure}

It is important to note that if only the middle section of the core was analysed, or a correction was applied to the saturation to remove the perceived impact of capillary end effects, the trapping curves are still dependent on the injection technique. The co-injection experiment has significantly higher trapping efficiency (although the initial gas saturation in lower). If co-injection experiments are conducted to estimate single phase injection, we are potentially heavily overestimating the amount of residual trapping in the subsurface, and underestimating the pore volume utilization. 

\subsection{Pressure and saturation evolution during drainage and imbibition}
\label{pressure}

The pressure drop across the core for the final 30 mins of the experiment is shown in Figure \ref{pressure_data}. The full pressure data is given in the Supplementary Material, but as we are focused on residual trapping, the final pressure response is of interest in this work. 

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.8\linewidth]{CHAPTERS/PICS/pressure.png}
	\end{center}
	\caption{The pressure drop across the core for the final 30 mins of injection. The blue lines show the pressure during imbibition and drainage for the co-injection experiment. The black lines show the pressure during imbibition and drainage for the single phase injection experiment. The pressure drop is higher during imbibition than drainage because trapped gas clusters increase resistance to flow.}
	\label{pressure_data}
\end{figure}

The differential pressure during drainage heavily depends on the injection technique. For co-injection drainage, the gas saturation is lower, and the differential pressure is higher. This implies more tortuous pathways for the gas, causing higher resistance to flow and subsequently higher pressure drop across the core. A greater proportion of the gas remains after imbibition for the co-injection experiment, suggesting that the more tortuous gas pathways encourage more residual trapping.

The pressure drop across the core is greater during imbibition, as trapped gas clusters create resistance to flow. During single phase imbibition, the pressure never plateaus. To understand the cause of this, we have to assess the evolution of the saturation with time. The saturation values during flow are less accurate than those acquired with flow stopped. This is due to fluid movement during the acquisition of an image (which takes 20s). However, the information  is useful for assessing the evolution in time (which we do for imbibition as the evolution timescales are much longer than for drainage). This is shown in Figure \ref{sat_evolution} for a) the co-injection experiment, and b) the single phase injection experiment. The red line denotes the gas saturation at the end of drainage. The gas saturation during imbibition is colour coded depending on the time the scan was acquired; a lighter colour denotes an earlier scan time i.e. earlier in the imbibition experiment.  

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=1.0\linewidth]{CHAPTERS/PICS/sat_evolution.png}
	\end{center}
	\caption{The saturation evolution during imbibition for a) the co-injection experiment and b) the single phase injection experiment. The red line denotes the gas saturation at the end of drainage. The gas saturation during imbibition is colour coded depending on the time the scan was acquired; a lighter colour denotes an earlier scan time i.e. earlier in the imbibition experiment. }
	\label{sat_evolution}
\end{figure}

The gas saturation close to the inlet is fairly constant, suggesting that the gas saturation dropping to zero at the outlet dominates the differential pressure measurement in Figure \ref{pressure_data}. This suggests that the pressure measurements, and associated relative permeability values, are potentially dominated by end effects, providing misrepresentative values for reservoir models. Even with end effects present during co-injection imbibition, the differential pressure plateaus. This suggests that end effects do not prevent the system reaching an equilibrium, and can manifest in the pressure data in subtle ways. These different pressure responses during imbibition suggest significantly different dynamics dependent on injection technique. 

Near the inlet the residual gas saturation is reached quickly. It is the region affected by capillary end effects that evolves slower. This suggests that the capillary end effects occur over longer timescales than other pore scale dynamics, and the length of the capillary end effect could be quantified by dS/dt. The gas saturation stabilises during imbibition quicker for the co-injection experiment, as shown in Figure \ref{sat_evolution} by more overlap at later times.

To explore timescales further, we transform the pressure data from Figure \ref{pressure_data} into the frequency domain in Figure \ref{FT_pressure}. The red dashed line denotes a slope of 1/$f^2$ i.e. red noise. This dashed line fits the imbibition data for both experiments, with the single phase imbibition power spectra having a larger amplitude, but the same slope as the co-injection imbibition power spectra. The slope showing red noise fits the longer timescales (smaller frequencies) during drainage, but the power spectra flattens out at the shorter timescales (large frequencies) to white noise. 

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=1.0\linewidth]{CHAPTERS/PICS/FT_pressure.png}
	\end{center}
	\caption{The pressure data transformed into the frequency domain for a) drainage and b) imbibition. The black lines denote single phase injection, and the blue lines denote co-injection. }
	\label{FT_pressure}
\end{figure}

Figure \ref{FT_pressure} shows that the co-injection drainage power spectra has a larger amplitude than the single-phase drainage power spectra. This is reversed during imbibition; with the single phase imbibition power spectra having a larger amplitude than co-injection imbibition power spectra. Both imbibition power spectra have a larger amplitude than the drainage power spectra. While there is a greater difference in the pressure difference across the core, and the saturation along the core, for the drainage sequence for both experiments, the power spectra have a more similar amplitude when compared to the imbibition sequence for both experiments where the saturation across the core are similar. The end effects evolve over longer timescales and, as shown in Figure \ref{FT_pressure}, the longer timescales have a larger amplitude in the power spectra, and thus are influencing the pressure data and relative permeability calculations more. This highlights the importance of understanding the manifestation of end effects in the pressure data and associated relative permeability values. 


\subsection{The role of heterogeneity on trapping efficiency}
By reversing the direction of flow, we are able to assess the impact of orientation of heterogeneity on flow properties for the different injection techniques. There are variations in saturation across the core (which are typical, even with repeat experiments with the core orientation kept the same). Full saturation results are given in the Supplementary Material.

The important difference is in the trapping curves in Figure \ref{trapping_curve_rev}. For the co-injection experiments, the trapping curve remains the same, regardless of core orientation. However, for the single phase experiments, the reversed core orientation leads to a different trapping curve, caused by the capillary end effects becoming more influential. This is likely due to the now slightly decreasing porosity with distance from the inlet; the porosity gradient is working in the same direction as the end effect, whereas for the initial orientation, the different effects were opposing each other. 

\begin{figure}[h]
	\begin{center}
		\centering
		\includegraphics*[angle=0, width=0.9\linewidth]{CHAPTERS/PICS/trapping_curve_rev.png}
	\end{center}
	\caption{The relationship between between initial gas saturation (post drainage) and residual gas saturation (post imbibition) for the co-injection experiment (black and blue crosses, the latter for the reversed core orientation) and single phase injection experiment (red and green circles, the latter for the reversed core orientation).}
	\label{trapping_curve_rev}
\end{figure}

The role of heterogeneity is dependent on the injection technique. 
This might be different for the oil experiments. 

\section{Conclusions}
Significant time and effort is used to measure relative permeability and residual trapping in rocks that are characteristic of the reservoir being used for carbon storage. To avoid capillary end effects, steady-state co-injection experiments are used to make measurements. In this work we show that the injection technique heavily influences the trapping efficiency, and this must be accounted for in future modelling efforts. Injection for CO$_2$ storage is typically single phase, meaning co-injection experiments might not be representative of what occurs in the subsurface. 

The orientation of heterogeneity was integral for single phase injection experiments. So the classification of heterogeneity and uncertainties related to heterogeneity will be more extreme with single phase injection. Furthermore without accounting for the complexity of flow, and how capillary end effects manifest in trapping relationships and pressure readings, the characterisation of the reservoir will be incorrect. While end effects were prevalent in both experiments, the behaviour during single phase injection cannot be predicted within the framework of the Land trapping model. 

Overall, the co-injection of water with gas improves trapping efficiency, even if end effects are excluded. But pore volume utilization is reduced, meaning that the CO$_2$ plume with spread out but more residual trapping will occur. An assessment of the trade-off between plume spread and residual trapping is required to understand if co-injection or alternating water and gas (WAG) is beneficial at the field scale. The experimental set-up influences the observations made, and this is something to be mindful of when upscaling observations. 

Further work is needed to assess the role of heterogeneity, and quantify the uncertainty of estimates caused by variations in heterogeneity. This should be explored for both carbonate, and sandstone samples. 


==> PREFACE/abstract.tex <==
\addcontentsline{toc}{chapter}{Abstract}
\begin{center}
\vspace*{0.5in}

\textbf{\Huge Abstract}
\vspace{0.5in}
\end{center}

\begin{abstract}
Multiphase flow in porous media has important implications in agriculture, carbon storage, groundwater contamination and oil recovery. The parameters that control the flow of immiscible fluids dictate the distribution of the fluids in the pore space and thus influence trapping and recovery. This report utilises both 2D glass micro-models and 3D natural rocks to explore the pore scale dynamics of two phase immiscible flow. 

\end{abstract}


==> PREFACE/acknowledgements.tex <==
\clearpage
\addcontentsline{toc}{chapter}{Acknowledgements}
\textbf{\Huge Acknowledgements}
\vspace{0.5in}

I would like to thank Ali Raeini for his network extraction code, Tom Bultreys for his help creating hexagons in MATLAB, Alessio Scanziani for his pore occupancy code, Lewis Lin and Ying Gao for their help in setting up the initial experiments in the micro-CT, Simon Franchini for showing me how to use the high speed camera for the micro-models, and Alessio Scanziani and Gaetano Garfi for their feedback on the content of this report. 

==> PREFACE/conventions.tex <==
\cleardoublepage

\addcontentsline{toc}{chapter}{Notation, Definitions and Conventions}

\vspace{2in}
\textbf{\Huge Notation, Definitions \& Conventions}

\section*{Symbols}

\begin{description}

\item[$V_P$] Primary wave speed
\item[$V_S$] Secondary wave speed
\item[$H$] Crustal thickness
\item[$\kappa$] Bulk crustal Vp/Vs ratio.
\item[$\sigma$] Poisson's ratio

\end{description}

\section*{Abbreviations}

\begin{description}

\item[RF] Receiver function

\item[Moho] Mohorovi\v{c}i\'{c} discontinuity

\end{description}

\section*{Conventions}

\begin{description}

\item[Backazimuth] The angle in degrees measured clockwise from north from a seismic station to the great circle arc between a seismic station and an earthquake.

\end{description}

==> README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
